Bug or not bug? That is the question

Nowadays, development teams often rely on tools such as Jira or Bugzilla to manage backlogs of issues to be solved to develop or maintain software. Although they relate to many different concerns (e.g., bug fixing, new feature development, architecture refactoring), few means are proposed to identify and classify these different kinds of issues, except for non mandatory labels that can be manually associated to them. This may lead to a lack of issue classification or to issue misclassification that may impact automatic issue management (planning, assignment) or issue-derived metrics. Automatic issue classification thus is a relevant topic for assisting backlog management. This paper proposes a binary classification solution for discriminating bug from non bug issues. This solution combines natural language processing (TF-IDF) and classification (multi-layer perceptron) techniques, selected after comparing commonly used solutions to classify issues. Moreover, hyper-parameters of the neural network are optimized using a genetic algorithm. The obtained results, as compared to existing works on a commonly used benchmark, show significant improvements on the F1 measure for all datasets.

==> Sections/longtable_results.tex <==
\newpage
\begin{landscape}

\onecolumn
%\resizebox{\textheight}{!}{

\begin{footnotesize}
\setlength\LTleft{0pt}
\setlength\LTright{0pt}
\begin{longtable}{@{\extracolsep{\fill}}|l|l|l|l|l|l|l|l|l|l|l|@{}}
\caption{Comparison of results obtained with different settings of our approach.}\\
\label{tab:results_intermediate}\\
\hline
Setting & Setting parameters & \multicolumn{8}{l|}{Results} & Evaluation Protocol       \\ \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2cm}}\textbf{Setting 1:}\\\textbullet\ Unigram only\\\textbullet\ No feature selection\\ \textbullet\ MLP by default\\ \textbullet\ No optimizations\end{tabular}} & 
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2.5cm}}\\\textbullet TfidfVectorizer(sublinear\_tf=False, ngram\_range=(1, 1)) \\ \textbullet MLPClassifier(random\_state=0)\end{tabular}} & 
\multicolumn{8}{c|}{\textbf{F1-Measure}} & \multirow{12}{*}{10-Fold} \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.711        & 95\% CI: 0.039      & 0.762       & 95\% CI: 0.069       & 0.736      & 95\% CI: 0.108     & \multirow{2}{*}{\textbf{0.748}} & \multirow{2}{*}{95\% CI: 0.058} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.736}}                                                       &                   &                           &                            \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Precision}}                                                                                                         &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.731        & 95\% CI: 0.070      & 0.778       & 95\% CI: 0.058       & 0.788      & 95\% CI: 0.127     & \multirow{2}{*}{\textbf{0.764}} & \multirow{2}{*}{95\% CI: 0.127} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.766}}                                                       &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Recall}}                                                                                                            &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.695        & 95\% CI: 0.084      & 0.748       & 95\% CI: 0.097       & 0.692      & 95\% CI: 0.106     & \multirow{2}{*}{\textbf{0.738}} & \multirow{2}{*}{95\% CI: 0.104}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean:0.712}}                                                        &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Accuracy}}                                                                                                          &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.769        & 95\% CI: 0.033      & 0.818       & 95\% CI: 0.047       & 0.858      & 95\% CI: 0.059     & \multirow{2}{*}{\textbf{0.827}} & \multirow{2}{*}{95\% CI: 0.052}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.815}}                                                        &                   &                           &                           \\ \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2cm}}\textbf{Setting 2:}\\\textbullet\ Uni-grams and bi-grams\\\textbullet\ No feature selection\\\textbullet\ Rare/Stop words dropping\\\textbullet\ Log function on term-frequency \\\textbullet\ MLP by default\\ \textbullet\ No optimizations\end{tabular}} & 
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2.5cm}}\\\textbullet TfidfVectorizer(max\_df=0.5, min\_df=2, sublinear\_tf=True, ngram\_range=(1, 2)) \\ \textbullet MLPClassifier(random\_state=0)\end{tabular}} & 
\multicolumn{8}{c|}{\textbf{F1-Measure}} & \multirow{12}{*}{10-Fold} \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.710       & 95\% CI: 0.102      & 0.762       & 95\% CI: 0.069       & 0.736      & 95\% CI: 0.108     & \multirow{2}{*}{\textbf{0.775}} & \multirow{2}{*}{95\% CI: 0.040} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.736}}                                                       &                   &                           &                            \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Precision}}                                                                                                         &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.747        & 95\% CI: 0.112      & 0.778       & 95\% CI: 0.058       & 0.788      & 95\% CI: 0.127     & \multirow{2}{*}{\textbf{0.816}} & \multirow{2}{*}{95\% CI: 0.133} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.766}}                                                       &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Recall}}                                                                                                            &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.679        & 95\% CI: 0.129      & 0.748       & 95\% CI: 0.097       & 0.692      & 95\% CI: 0.106     & \multirow{2}{*}{\textbf{0.745}} & \multirow{2}{*}{95\% CI: 0.096}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean:0.712}}                                                        &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Accuracy}}                                                                                                          &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.773        & 95\% CI: 0.078      & 0.818       & 95\% CI: 0.047       & 0.858      & 95\% CI: 0.059     & \multirow{2}{*}{\textbf{0.849}} & \multirow{2}{*}{95\% CI: 0.041}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.815}}                                                        &                   &                           &                           \\ \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2cm}}\textbf{Setting 3:}\\\textbullet\ Uni-grams and bi-grams\\\textbullet\ Rare/Stop words dropping\\\textbullet\ Log function on term-frequency \\ \textbullet\ Feature selection with Chi2 (20000)\\ \textbullet\ MLP by default\\ \textbullet\ No optimizations\end{tabular}} & 
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2.5cm}}\textbullet\ 20000 features \\\textbullet TfidfVectorizer(max\_df=0.5, min\_df=2, sublinear\_tf=True, ngram\_range=(1, 2)) \\ \textbullet MLPClassifier(random\_state=0)\end{tabular}} & 
\multicolumn{8}{c|}{\textbf{F1-Measure}} & \multirow{12}{*}{10-Fold} \\ \cline{3-10}    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.778        & 95\% CI: 0.099      & 0.861       & 95\% CI: 0.045       & 0.850      & 95\% CI: 0.075     & \multirow{2}{*}{\textbf{0.859}} & \multirow{2}{*}{95\% CI: 0.037} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.830}}                                                       &                   &                           &                            \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Precision}}                                                                                                         &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.887        & 95\% CI: 0.135      & 0.918       & 95\% CI: 0.057       & 0.924      & 95\% CI: 0.065     & \multirow{2}{*}{\textbf{0.916}} & \multirow{2}{*}{95\% CI: 0.089} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.910}}                                                       &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Recall}}                                                                                                            &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.695        & 95\% CI: 0.109      & 0.812       & 95\% CI: 0.064       & 0.789      & 95\% CI: 0.118     & \multirow{2}{*}{\textbf{0.811}} & \multirow{2}{*}{95\% CI: 0.055}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean:0.765}}                                                        &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Accuracy}}                                                                                                          &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.838        & 95\% CI: 0.074      & 0.898       & 95\% CI: 0.032       & 0.921      & 95\% CI: 0.037     & \multirow{2}{*}{\textbf{0.907}} & \multirow{2}{*}{95\% CI: 0.052}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.886}}                                                       &                   &                           &                           \\ \hline \\
        \pagebreak
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2cm}}\textbf{Setting 4:}\\\textbullet\ Uni-grams and bi-grams\\\textbullet\ Rare/Stop words dropping\\\textbullet\ Log function on term-frequency \\ \textbullet\ Feature selection with Chi2 (20000)\\ \textbullet\ MLP parameters optimized with Grid-Search\\ \end{tabular}} & 
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2.5cm}}\textbullet\ 20000 features \\\textbullet TfidfVectorizer(max\_df=0.5, min\_df=2, sublinear\_tf=True, ngram\_range=(1, 2)) \\ \textbullet MLPClassifier(activation='tanh', learning\_rate='adaptive', max\_iter=100, random\_state=0)\end{tabular}} & 
\multicolumn{8}{c|}{\textbf{F1-Measure}} & \multirow{12}{*}{10-Fold} \\ \cline{3-10}    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.777        & 95\% CI: 0.099      & 0.858       & 95\% CI: 0.048       & 0.846      & 95\% CI: 0.083     & \multirow{2}{*}{\textbf{0.858}} & \multirow{2}{*}{95\% CI: 0.035} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.830}}                                                       &                   &                           &                            \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Precision}}                                                                                                         &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.887        & 95\% CI: 0.135      & 0.915       & 95\% CI: 0.054       & 0.934      & 95\% CI: 0.049     & \multirow{2}{*}{\textbf{0.916}} & \multirow{2}{*}{95\% CI: 0.082} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.910}}                                                       &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Recall}}                                                                                                            &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.695        & 95\% CI: 0.109      & 0.809       & 95\% CI: 0.070       & 0.776      & 95\% CI: 0.140     & \multirow{2}{*}{\textbf{0.809}} & \multirow{2}{*}{95\% CI: 0.060}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean:0.765}}                                                        &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Accuracy}}                                                                                                          &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.838        & 95\% CI: 0.074      & 0.896       & 95\% CI: 0.034       & 0.920      & 95\% CI: 0.038     & \multirow{2}{*}{\textbf{0.907}} & \multirow{2}{*}{95\% CI: 0.025}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.886}}                                                       &                   &                           &                           \\ \hline
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2cm}}\textbf{Setting 5:}\\\textbullet\ Uni-grams and bi-grams\\\textbullet\ Rare/Stop words dropping\\\textbullet\ Log function on term-frequency \\ \textbullet\ Feature selection with Chi2 \\ \textbullet\ Feature number optimized with GA (24954) \\\textbullet\ MLP parameters optimized with Grid-Search and GA\\ \end{tabular}} & 
\multirow{12}{*}{\begin{tabular}[c]{@{}p{2.5cm}}\textbullet\ 24954 features \\\textbullet TfidfVectorizer(max\_df=0.5, min\_df=2, sublinear\_tf=True, ngram\_range=(1, 2)) \\ \textbullet MLPClassifier(activation='tanh', learning\_rate='adaptive', max\_iter=100, hidden\_layer\_sizes=(8, 13, 18, 14, 11), random\_state=0)\end{tabular}} & 
\multicolumn{8}{c|}{\textbf{F1-Measure}} & \multirow{12}{*}{10-Fold} \\ \cline{3-10}    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.807        & 95\% CI: 0.084      & 0.875       & 95\% CI: 0.032       & 0.862      & 95\% CI: 0.081     & \multirow{2}{*}{\textbf{0.869}} & \multirow{2}{*}{95\% CI: 0.065} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.830}}                                                       &                   &                           &                            \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Precision}}                                                                                                         &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.888        & 95\% CI: 0.115      & 0.908       & 95\% CI: 0.052       & 0.924      & 95\% CI: 0.063     & \multirow{2}{*}{\textbf{0.921}} & \multirow{2}{*}{95\% CI: 0.106} &      \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.910}}                                                       &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Recall}}                                                                                                            &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.741        & 95\% CI: 0.098      & 0.845       & 95\% CI: 0.040       & 0.811      & 95\% CI: 0.132     & \multirow{2}{*}{\textbf{0.828}} & \multirow{2}{*}{95\% CI: 0.117}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean:0.765}}                                                        &                   &                           &                           \\ \cline{3-10}
    &                    & \multicolumn{8}{c|}{\textbf{Accuracy}}                                                                                                          &                           \\ \cline{3-10}
    &                    & \multicolumn{2}{l|}{HTTPClient} & \multicolumn{2}{l|}{Jackrabbit} & \multicolumn{2}{l|}{Lucene} & \multicolumn{2}{l|}{\textbf{Cross-project}}            &                           \\ \cline{3-10}
    &                    & 0.855        & 95\% CI: 0.062      & 0.906       & 95\% CI: 0.024       & 0.927      & 95\% CI: 0.039     & \multirow{2}{*}{\textbf{0.914}} & \multirow{2}{*}{95\% CI: 0.043}  &     \\ \cline{3-8}
    &                    & \multicolumn{6}{c|}{\textbf{Mean: 0.886}}                                                       &                   &                           &                           \\ \hline \\
\end{longtable}%}
\end{footnotesize}
\twocolumn
\end{landscape}


